Hybrid Automata for Formal Modeling and Verification of Cyber-Physical Systems

The presence of a tight integration between the discrete control (the "cyber") and the analog environment (the "physical")---via sensors and actuators over wired or wireless communication networks---is the defining feature of cyber-physical systems. Hence, the functional correctness of a cyber- physical system is crucially dependent not only on the dynamics of the analog physical environment, but also on the decisions taken by the discrete control that alter the dynamics of the environment. The framework of Hybrid automata---introduced by Alur, Courcoubetis, Henzinger, and Ho---provides a formal modeling and specification environment to analyze the interaction between the discrete and continuous parts of a cyber-physical system. Hybrid automata can be considered as generalizations of finite state automata augmented with a finite set of real-valued variables whose dynamics in each state is governed by a system of ordinary differential equations. Moreover, the discrete transitions of hybrid automata are guarded by constraints over the values of these real-valued variables, and enable discontinuous jumps in the evolution of these variables. Considering the richness of the dynamics in a hybrid automaton, it is perhaps not surprising that the fundamental verification questions, like reachability and schedulability, for the general model are undecidable. In this article we present a review of hybrid automata as modeling and verification framework for cyber-physical systems, and survey some of the key results related to practical verification questions related to hybrid automata.

==> algorithms.tex <==
\begin{algorithm}[t]
  \KwIn{A finite automaton $\Hh(P)$ and property $\phi {\in} \LTL(P)$}
  \KwOut{Yes, if $\Aa$ satisfies $\phi$ and No, otherwise.}
  $\Aa_{\neg\phi}(\set{p}) := $ Finite automata corresponding to the negation of
  the LTL property $\phi$\;
  $\Hh' := \Hh(P) \otimes \Aa_{\neg\phi}(\set{p})$\;
  
  \If {$\Gee\Eff(\Hh', p)$ = Yes} 
  {
    \Return No\;
  }
  \Else { 
    \Return Yes\; 
  }
  \caption{$\textsc{ModelCheck}(\Hh,\phi)$}
  \label{ModelCheckingFA}
\end{algorithm}

\begin{algorithm}[t]
  \KwIn{A hybrid automaton $\Hh = (S, S_0, \Sigma, \Delta, P, L)$ and target set
    $T  \in S$} 
  \KwOut{Return the set of all states of $\Hh$ that can reach a state in $T$.}
  $S_\text{curr} := \emptyset$\;
  $S_\text{next} := T$\;
  
  \While {$S_\text{curr} \not = S_\text{next}$} 
  {
    $S_\text{curr} := S_\text{next}$\;
    $S_\text{next} := S_\text{next} \cup \set{s \in S \::\: \exists 
      s' {\in} S_\text{next}, \exists a {\in} \Sigma\text{ s.t. }
      (s, a, s') \in \Delta}$\;
  }
  \Return $S$\;
  
  \caption{$\textsc{Reach}(\Hh, T)$}
  \label{Reachability}
\end{algorithm}

\begin{algorithm}[t]
  \KwIn{A hybrid automaton $\Hh= (S, S_0, \Sigma, \Delta, P, L)$ and safety set
    $T$} 
  \KwOut{Return the set of all states of $\Hh$ from where $\Hh$ has an
    infinite run that only visit states in $T$}
  $S_\text{curr} := \emptyset$\;
  $S_\text{next} := T$\;
  
  \While {$S_\text{curr} \not = S_\text{next}$} 
  {
    $S_\text{curr} := S_\text{next}$\;
    $S_\text{next} := \set{s \in S_\text{next} \::\: \exists s' {\in}
      S_\text{next}, \exists a {\in} \Sigma  
      (s, a, s') \in \Delta}$\;
  }
  \Return $S$\;
  
  \caption{$\textsc{Safety}(\Hh, T)$}
  \label{Safety}
\end{algorithm}

\begin{algorithm}[t]
  \KwIn{A hybrid automaton $\Hh(P)$ and proposition $p \in P$}
  \KwOut{Yes, if there is a trace of $\Hh$ that visit a $p$-labeled state
    infinitely often and No, otherwise.}
  Let $\sem{\Hh} = (S, S_0, \Sigma, \Delta, P, L)$ be the state transition graph
  of $\Hh$\; 
  
  $T := \set{s \::\: L(s) = p}$\;
  
  
  \If {$S_0 \cap (\textsc{Safety}(\Hh, \textsc{Reach}(\Hh, T))) \not = \emptyset$} 
  {
    \Return Yes\;
  }
  \Else { 
    \Return No\; 
  }
  \caption{$\Gee\Eff(\Hh, p)$}
  \label{GFp}
\end{algorithm}


==> finiteBisimulation.tex <==
In this section we introduce the concept of bisimulation relation between two
Kripke structures, and show that for two bisimilar systems (systems having a
bisimulation relation between their states) we have that both systems 
have the same set of traces, and hence precisely the same set of LTL formulas
are satisfied by both of them.
Using this idea, we show that if for a given hybrid Kripke structure $\Hh$ there
exists a bisimulation relation with some finite state Kripke structure $\Kk$,
then the problem of LTL model-checking for $\Hh$ can be reduced to the decidable
problem of LTL model-checking for finite Kripke structure $\Kk$.

%Kripke structures are useful for modelling software/hardware systems at various levels 
%of abstraction. If the level of abstraction is low, then the transition system 
%has a lot of implementation details; on the other  hand, if the level of abstraction is high, then 
%there will be fewer implementation details. Consider a piece of software that models
%a remote control system which controls three race cars $C_1, C_2, C_3$. 
%Before reaching the finish line, a bridge has to be crossed. The bridge can carry exactly one car 
%at any point of time, an overload may cause a bridge collapse. 
%Assume that we use 3 boolean variables $x,y,z$ to denote the cars that  
%are currently on the bridge.  A safety requirement to be enforced is that atmost one of $x,y,z$ can be 1. 
%A low level abstraction $L$ can model the situation that from any of the states $x=1, y=0,z=0$ or 
%$x=0,y=1,z=0$ or $x=y=0,z=1$, the finish line can be reached. A higher level of abstraction 
%$H$ can simply say that the finish line can be reached whenever $x \wedge y \wedge z=0$. 
%Note that $H$ allows for unsafe behaviours : for instance, $x=y=1,z=0$ is allowed by $H$.  
%$L$ can be obtained by refining $H$; that is, by adding more implementation details. Similarly, $H$ can be obtained 
%from $L$ by hiding a few implementation details. 

%Bisimulation relations are used for comparing two models of the same system, 
%or for checking whether a system model satisfies a specification. 
%Consider a Kripke structure $(\Hh, P, L)$ that is an abstraction of some system
%specification, and also consider a more detailed structure $(\Hh', P, L')$.  
%Bisimulation relations provides techniques to abstract away  details that are
%irrelevant for the analysis of a given property $\phi$. 
%This can be used to obtain a smaller model $(\Hh, P, L)$ from a very large model
%$(\Hh', P, L')$, provided the abstraction preserves the property $\phi$. 
%In this case, checking $\Hh \models \phi$ is sufficient to check if $\Hh'
%\models \phi$.  

We say that a Kripke structure $\Kk' = (\Tt', P, L')$ can \emph{simulate} a Kripke
structure $\Kk'= (\Tt, P, L)$ if every step of $\Kk$ can be matched (with 
respect to atomic propositions) by one or more steps of $\Kk'$.
A Bisimulation equivalence denotes the presence of a mutual simulation between
two structures $\Kk$ and $\Kk'$.
Formally, bisimulation relation in the following manner.
%
\begin{definition}[Bisimulation Relation]
  Let $\Kk = (\Tt = (S, S_0, \Sigma, \Delta), P, L)$ and $\Kk' = (\Tt = (S',
  S_0', \Sigma', \Delta'), P, L')$ be two Kripke structures.
  A bisimulation relation between $\Kk$ and $\Kk'$ is a binary relation $\Rr
  \subseteq S \times S'$ such that: 
  \begin{itemize}
  \item 
    every initial state of $\Tt$ is related to some initial state of $\Tt'$,
    and vice-versa, i.e. for every $s \in S_0$  there exists $s' \in S_0'$ such
    that $(s, s') \in \Rr$ and for every $s' \in S_0'$ there exists a $s \in
    S_0$ such that $(s, s') \in \Rr$;
  \item 
    for every $(s, s') \in {\mathcal R}$ the following holds:
    \begin{itemize}
    \item 
      $L(s)=L'(s')$,
    \item 
      every outgoing transition of $s$ is matched with some outgoing
      transition of $s'$, i.e. if $t \in \post(s)$ then there exists 
      $t' \in \post(s')$ with $(t, t') \in \Rr$, and  
    \item 
      every outgoing transition of $s'$ is  matched with some outgoing
      transition of $s$, i.e. if $t' \in \post(s')$ then there exists 
      $t \in \post(s)$ with $(t, t') \in \Rr$. 
    \end{itemize}
  \end{itemize}
\end{definition}
We say that $\Tt$ and $\Tt'$ (analogously, $\Kk$ and $\Kk'$) are bisimilar or
bisimulation equivalent, and we write $\Tt \sim \Tt'$, if there exists a
bisimulation relation $\Rr \subseteq S \times S'$. 

%\begin{example}
%  Figure \ref{bisim1} gives two transition systems which are not bisimilar. 
%  \input{bisim1.tex}
%  The transition systems in figure \ref{bisim1} model the flights of two
%  airlines. 
%  It is clear that for the first airline, it is possible to reach Shimla and
%  Delhi from Mumbai on  any day;  
%  the airline on the right however, has exactly one choice of destination from
%  Mumbai on any given day.  
%\end{example}

The following Proposition follows from the definition of bisimulation and the
semantics of LTL.
\begin{proposition}
  \label{trace-eq}
  If $\Tt \sim \Tt'$ then $\Trace(\Tt)=\Trace(\Tt')$.
  Moreover, if $\Tt \sim \Tt'$ then for every LTL formula $\phi$ we have that 
  $\Tt \models \phi$ if and only if $\Tt' \models \phi$.
\end{proposition}
\begin{proof}
  Let $\Tt \sim \Tt'$. 
  Using a simple inductive argument, one can show that for every run $a = \seq{s_0,
    a_1, s_1, a_2, \ldots}$ of $\Tt$ there is a run $r' = \seq{s_0', a_1', s_1', a_2',
    \ldots}$ of $\Tt'$ such that $L(s_i) = L'(s_i')$ for every $i \geq 0$.
  This implies that $\Trace(r) = \Trace(r')$ and hence $\Trace(\Tt) \subseteq
  \Trace(\Tt')$. 
  Similarly, we can show that $\Trace(\Tt') \subseteq \Trace(\Tt)$.
  Hence it follows that $\Tt \sim \Tt'$ implies  $\Trace(\Tt)=\Trace(\Tt')$.
  To prove the other part of the proposition, observe 
  % that two trace equivalent
  % structures $\Tt$ and $\Tt'$ always satisfy the same LTL formulae, since  
  %both have exactly the same set of traces, and 
  LTL formulae are interpreted over traces of structures, and since two
  bisimilar Kripke structures have the same set of traces, it follows that for
  every LTL formula $\phi$ we have that $\Tt \sim \Tt'$ implies that 
  $\Tt \models \phi$ if and only if $\Tt' \models \phi$.
\end{proof}
This proposition shows that LTL model checking problem can be reduced to solving
LTL model checking problem over a bisimilar Kripke structure.
We next show how to extend this idea to define bisimulation over the states of a
Kripke structure, and use it to produce a bisimilar Kripke structure with fewer
states. 
%
\begin{definition}[Bisimulation Relation on $\Kk$]
  Let $\Kk=(\Tt=(S, S_0, \Sigma, \Delta), P, L)$ be a Kripke structure. 
  A bisimulation on $\Kk$ is a binary relation $\Rr \subseteq S \times S$ such
  that for all $(s, s') \in \Rr$ we have that:
  \begin{itemize}
  \item 
    $L(s)=L(s')$;
  \item 
    if $t \in \post(s)$, then there exists an $t' \in \post(s')$ such that $(t,
    t') \in \Rr$; 
 \item 
   if $t' \in \post(s')$, then there exists an $t \in \post(s)$ such that $(s',
   t') \in \Rr$. 
\end{itemize}
\end{definition}
% 
It is easy to see that a bisimulation relation $\Rr$ over the state space of
$\Kk$ is an equivalence relation. 
For a state $s \in S$ we write $[s]_\Rr$ for the equivalence class of $\Rr$
containing $s$.
We say that states $s, s' \in S$ are bisimulation equivalent, and we write 
$s \sim_{\Tt} s'$, if there exists a bisimulation relation $\Rr$ for $\Tt$ 
with $(s, s') \in \Rr$. 

Given a Kripke structure $\Tt$, we use a bisimulation relation $\Rr$ for
reducing the state space of $\Tt$ using the following quotient construction. 
\begin{definition}[Bisimulation Quotient]
  Given a Kripke structure $\Kk = (\Tt=(S, S_0, \Sigma, \Delta), P, L)$ and a
  bisimulation relation $\Rr \subseteq S \times S$ over $\Kk$, the bisimulation
  quotient $\Kk_\Rr$ is defined as a Kripke structure 
  $\Kk_\Rr=(\Tt_\Rr=(S_\Rr, S^0_{\Rr}, \Sigma_\Rr, \Delta_\Rr), P, L_\Rr)$
  where: 
  \begin{itemize}
  \item 
    the state space of $\Tt_\Rr$ is the quotient space of $\Tt$, i.e. 
    $S_\Rr = \set{[s]_\Rr \::\: s \in S}$;
  \item  
    the set of initial states is the set of $\Rr$-equivalence classes of the
    initial states, i.e. $S^0_\Rr=\set{[s]_\Rr \::\: s \in S_0}$;
  \item 
    $\Sigma_\Rr = \set{\tau}$;
  \item 
    Each transition $(s,a,s') \in \Delta$ induces a transition from $[s]_{\Rr}$
    to $[s']_{\Rr}$ in $\Delta_\Rr$, i.e. 
    $\Delta_\Rr=\set{([s]_\Rr, \tau, [s']_\Rr) \::\: (s, \alpha, s') \in
      \Delta}$, and
  \item 
    $L_\Rr$ is defined such that $L_\Rr([s]) = L(s)$~\footnote{Observe that the
      definition of bisimulation ensures that the state labeling $L_\Rr$ is well
      defined.}.
  \end{itemize}
\end{definition}
%  Note that for model checking purposes, we only need the traces 
%  of the transition system; the actions play no role. 
%  We now give an example to see the state space reductions possible by quotienting. 
%  Consider the situation at an airport with $n$ aircrafts at bay. 
%  Each aircraft is one of the two states : ready for take-off or 
%  not ready for take-off. Modeling this as a transition system $TS$, 
%  with $S=\{(a_1,a_2, \dots, a_n) \mid a_i \in \{0,1\}\}$, 
%  we have states corresponding to all $n$-tuples
%  of possibilities of aircraft $i$ being ready for take-off or not. 
%  However, intuitively, $L(s)$ denotes the number of aircrafts 
%  that are ready for take-off at any point of time. 
%  Figures \ref{q1}, \ref{q2} shows the system before and after quotienting for the case 
%  of $n=3$. 
%  
%  \input{q1}
%  \input{q2}
%




==> oldHA.tex <==


%PTIME membership of reachability and schedulability problems, undecidability by
%introducing either local invariant or guards, or a single clock
%variable. Connection with timed automata with energy variables. 

%bounded-rate decidability..

%Integration graphs and Hybrid systems with piecewise-constant derivatives (PCD)
%decidability for planar grpahs, undecidability for 3 dimension, PCD with n
%variables and arithmetical hierarchy

%Introducing clocks to MMS energy games... 


%\subsection{Classification of Hybrid Automata}
%Before we present a classification of hybrid automata, we distinguish between
%different kind of variables. 
%Let us fix a hybrid automaton $\Hh = (M, M_0, \Sigma, X, \Delta, I,F, V_0)$.  
%We classify the variables based on its flow function $F$.
%We say that a variable $x \in X$ is \emph{linear} if for all $m \in M$ we have 
%that $F(m)(x)$ is a polyhedral predicate. 
%\begin{definition}[LHA]
%  A \emph{linear hybrid automaton} is a hybrid automaton $\Hh = (M, M_0, \Sigma,
%  X, \Delta, I,F, V_0)$ such that: 
%  \begin{itemize}
%  \item
%    all variables in $X$ are linear;
%  \item 
%    for all $(m, g, a, r, m') \in \Delta$ we have that $g$ and $r$ are
%    polyhedral predicates;
%  \item 
%    for all $m \in M$ the predicate $I(m)$ is polyhedral; and
%  \item 
%    the predicate $V_0$ is polyhedral. 
%  \end{itemize} 
%\end{definition}

%We say that a variable $x \in X$ is \emph{rectangular} if for all $m
%\in M$ we have that $F(m)(x)$ is an interval. 
%\begin{definition}[RHA]
%  A \emph{rectangular hybrid automaton} is a hybrid automaton $\Hh = (M, M_0, \Sigma,
%  X, \Delta, I,F, V_0)$ such that: 
%  \begin{itemize}
%  \item 
%    all variables in $X$ are rectangular;
%  \item 
%    for all $(m, g, a, r, m') \in \Delta$ we have that $g$ and $r$ are
%    rectangular predicates;
%  \item 
%    for all $m \in M$ the predicate $I(m)$ is rectangular; and
%  \item 
%    the predicate $V_0$ is rectangular. 
%  \end{itemize} 
%\end{definition}
%We say that a rectangular hybrid automaton is \emph{initialized} if for every
%transition $(m, g, a, r, m') \in \Delta$ we have that for every variable $x \in
%X$ if $R(m)(x) \not = R(m')(x)$ then $r$.

%Lazy rectangular hybrid automata ...

%Similarly, we say that a variable if \emph{singular} if for all $m
%\in M$ we have that $F(m)(x)$ is a constant.  

%A singular variable $x \in X$ is called a \emph{clock} if $F(m)(x)=1$ for all
%modes $m \in M$. 
%Generalizing the concept of a clock, we call a variable \emph{skewed clock} if
%there exists a $K \in \Rplus$ such that $F(m)(x)=K$ for all modes $m \in M$. 
%We call a singular variable \emph{two-slope} if there are two distinct $k, k'
%\in \Rplus$ such that for all modes $m\in M$ we have that either $F(m)(x) = k$
%or $F(m)(x) = k'$; moreover if $k=0$ and $k'=1$ then we call the 
%two-slop variable a \emph{stopwatch}.
%Finally, we call a variable $x$ a \emph{memory cell} if its value does not
%change inside a mode, i.e.,  $F(m)(x) = 0$ for all modes $m \in M$. 


%\begin{definition}[Timed Automata]

%\end{definition}


%\begin{definition}[Singular Automata]

%\end{definition}

%\begin{definition}[Constant-Rate Multi-mode Systems]

%  ...and bounded-rate 
%  ... Constant-slope hybrid systems.. 
%  ... Integration Graphs...
%  ... clocks and energy automata... 
%\end{definition}

%\begin{definition}[PCD Systems]


%\end{definition}

% A function $dif$ mapping each element of $V \times L$ to an activity constraint. 
% An activity constraint on a variable $x \in V$ is either a differential equation in $x$
% or a statement of the form $\dot{x} \in [a,b]$ where $a,b$ are integers. 
% \item A finite set $E$ of edges. An edge is of the form 
% $(l,l',\varphi,R)$, where $l, l'$ are modes, $\varphi$ is a predicate called 
% the enabling condition, and  $R$ is a variable assignment called the reset condition. 
% A predicate in its most general form looks like 
% $a_1 x_1 + \dots + a_n x_n \sim b_1 y_1 + \dots + b_m y_m$, where 
% $a_i, b_j \in \mathbb{Z}, \sim \in \{<, \leq, =, >, \geq,\neq\}$ and $x_i, y_j
% \in V$. 

%A variable assignment 
%can be of one of the following forms:\\
% (i) Reset assignment : A variable $x$ is assigned 0.\\
% (ii) Variable-to-variable assignment : A variable $x$ is assigned the value of another variable $y$.
%Occasionally, it is convenient to assign invariants to modes. Mode invariants are predicates which 
%must be satisfied whenever the control resides at the mode.

%Given a hybrid automaton $H=(L, L_0, V, dif, E)$, we classify the variables 
%based on the activity constraints imposed by $dif$. 
%\begin{enumerate}
% \item A variable $x$ is called a {\it clock} iff for each $l \in L$, $dif(x,l)=1$.
% \item A variable $x$ is called a {\it skewed clock} iff there exists some $g \in {\mathbb R}_{+}$ with $g \neq 0,1$
%such that for each $l \in L$, $dif(x,l)$ is $\dot{x}=g$.
%\item  A variable $x$ is called a {\it memory cell} iff for each $l \in L$, $dif(x,l)$ is $\dot{x}=0$.
%\item  A variable $x$ is called a {\it stopwatch} iff for each $l \in L$,  $dif(x,l)$ is either $\dot{x}=0$ 
%or $\dot{x}=1$.
%\item A variable $x$ is called a {\it two-slope variable} iff there exists $g, h \in {\mathbb R}_{+}$, $g \neq h$ 
%such that for each $l \in L$,  $dif(x,l)$ is either $\dot{x}=g$  or $\dot{x}=h$.
%\item A variable $x$ is called  {\it linear} iff for each $l \in L$, there exists an interval $[a,b]$
%such that  $dif(x,l)$ is $\dot{x} \in [a,b]$.
%\end{enumerate}

A hybrid automaton in which all the variables are clocks is a timed automaton. 

%\subsection{Semantics}
%Let $H=(L, L_0, V, dif, E)$ be a hybrid automaton. A state is a pair $(l, \nu)$ consisting of a mode $l \in L$ and a 
%valuation $\nu \in {\mathbb{R}}^{|V|}$. 
%We define two kinds of successors of a state : (i) delay successor and (ii) edge successor.\\

%\noindent{\bf Edge Successor}: $(l,\nu) \vartriangleright (l', \nu')$ iff there exists some edge 
%$e=(l,l',\varphi,R)$ such that $\nu \models \varphi$ and $\nu'$ is obtained by 
%applying the reset assignment $R$. 

%\noindent{\bf Delay Successor}: $(l,\nu) \longrightarrow (l, \nu')$ iff there exists a 
%time delay $t \geq 0$ such that for each $x \in V$, a function $f_x: [0,t] \rightarrow {\mathbb R}$ such that 
%\begin{itemize}
% \item $f_x(0)=\nu(x), f_x(t)=\nu'(x)$,
% \item $f_x$ satisfies $dif(x,l)$. This is easy to see if $dif(x,l)$ is a differential equation. 
% If $dif(x,l)$ is of the form $\dot{x} \in [a,b]$, then 
% we must have $\dot{f_x(t')} \in [a,b]$ for each $t' \in (0,t)$, and similarly 
% for the left and right derivatives of $f_x$ at 0 and $t$ respectively. 
% \end{itemize}

%A computation of $H$ is a sequence $(l_n, \nu_n)_{n \in \omega}$ of states
%$(l_0,\nu_0) \longrightarrow (l_1, \nu_1) \longrightarrow (l_2, \nu_2) \dots$ such that $l_0 \in L_0$,
% $\nu_0(x)=0$ for all $x \in V$, and for each $i \in \mathbb{N}$, either 
% $(l_i, \nu_i) \vartriangleright (l_{i+1}, \nu_{i+1})$ or 
% $(l_i, \nu_i) \longrightarrow (l_{i+1}, \nu_{i+1})$. 
 
% The reachability problem for hybrid automata is stated as follows: Given a hybrid automaton ${\mathcal H}$ and a 
% state $(l,\nu)$, does there exist a computation of $H$ and a $j \in \mathbb{N}$ such that 
% $(l_j, \nu_j)=(l,\nu)$. 

 \begin{lemma}
\label{reach}
Given a hybrid automaton ${\mathcal H}$, a configuration $(l,\nu)$ is reachable in $H$ 
iff it is reachable in the transition system $T^{\mathcal H}$.
\end{lemma}



==> oldprelimx.tex <==
\subsection{Notation}
%\input{constraints}

Let $\Real$ be the set of real numbers, $\Rplus$ be the set of non-negative
real numbers, and $\Int$ be the set of integers. 


{\bf Valuations, Points, and Vectors.} 
Let $X$ be a set of real-valued variables. 
A \emph{valuation} on $X$ is a function $\nu : X {\to} \Rplus$ and we write $V(X)$
for the set of valuations on $X$.
If $|X| = n$ then, abusing notation, we also treat a valuation $\nu$ as a point in
$\Real^n$ that is equipped with the standard \emph{Euclidean norm}
$\norm{\cdot}$. 
We denote points (valuations) in this valuation space by $\pp, \pq$ and  vectors
by $\vr, \vv$.
We denote the $i$-th coordinate of point $\pp$ and vector $\vr$ by
$\pp(i)$ and $\vr(i)$, respectively.
Similarly, for a variable $x \in X$ we denote the coordinate of point $\pp$ and
vector $\vr$ corresponding to $x$ by $\pp(x)$ and $\vr(x)$, respectively.
We write $\vzero$ for a vector with all its coordinates equal to $0$; 
its dimension is often clear from the context.
The distance $\norm{\pp, \pq}$ between points $\pp$ and $\pq$ is defined as
$\norm{\pp - \pq}$. 
For two vectors ${\vv_1, \vv_2 \in \Real^n}$, we write $\vv_1 \dotprod \vv_2$
to denote their dot product defined as $\sum_{i=1}^n \vv_1(i)\cdot\vv_2(i)$.


\noindent{\bf Boundedness and Interior.} 
We denote a {\em closed ball} of radius $d \in \Rplus$ centered at $\pp$ as
$\ball{d}{\pp} {=} \set{\pq {\in} \Real^n \::\: \norm{\pp,\pq} \leq d}$.
We say that a set $S \subseteq \Real^n$ is {\em bounded} if there exists
$d \in \Rplus$ such that for all $\pp, \pq \in S$ we have
$\norm{\pp,\pq} \leq d$.
The {\em interior} of a set $S$, $\interior(S)$, is the set of all points
$\pp \in S$ for which there exists $d > 0$ s.t. $\ball{d}{\pp} \subseteq S$.

\noindent{\bf Convexity.} A point $\pp$ is a \emph{convex
  combination} of a finite set of points $P = \set{\pp_1, \pp_2, \ldots, \pp_k}$ if
there are $\lambda_1, \lambda_2, \ldots, \lambda_k \in [0, 1]$ such that
$\sum_{i=1}^{k} \lambda_i = 1$ and $\pp = \sum_{i=1}^k \lambda_i \cdot \pp_i$.
The \emph{convex hull} $\CVH{S}$ of a set $S$ is then the set of all points
that are convex combinations of points in $S$.
We say that $S \subseteq \Real^n$ is {\em convex} iff for all
$\pp, \pq \in S$ and all $\lambda \in [0,1]$ we have
$\lambda \pp + (1-\lambda) \pq \in S$ and moreover,
$S$ is a {\em convex polytope} if it is bounded and there exists $k \in \Nat$, a
matrix $A$ of  size $k \times n$ and a vector $\vb \in \Real^k$ such that $\pp
\in S$ iff $A\pp \leq \vb$. 
We write $\rows{M}$ for the number of rows in a matrix $M$, here $\rows{A}=k$. 
%Such \emph{hyperplane}-based representation of a convex-polytope is also known
%as an $\Hh$-representation. 
Convex polytopes can also be represented using the notion of a vertex.
A point $\pp$ is a \emph{vertex} of a convex polytope $P$ if it is
not a convex combination of two distinct (other than $\pp$) points in $P$. 
For a convex polytope $P$ we write $\Vtx{P}$ for the finite set of points that
correspond to the vertices of $P$.  
Each point in $P$ can be written as a convex combination of the points in
$\Vtx{P}$, or in other words, $P$ is the \emph{convex hull} of $\Vtx{P}$. 
%Hence a polytope can be equivalently represented as the set of its vertices: we
%call such representation a $\Vv$-representation. 
%Motzkin showed in 1930 that for each polytope given as an $\Hh$-representation,
%the convex hull of its vertices defines the polytope given as a
%$\Vv$-representation, and for each polytope given as a $\Vv$-representation the
%corresponding $\Hh$-representation can be given by computing the half-spaces
%defined by its facets.

%\noindent{\bf Union, Intersection, and Membership.}
%Given two sets $S_1, S_2 \in \Real^n$ their union $S_1 \cup S_2$ is defined as
%\[ 
%S_1 \cup S_2 \rmdef \set{\pp \::\: \pp \in S_1 \text{ or } \pp \in S_2}.
%\] 
%Similarly, for the intersection $S_1 \cap S_2$ of the sets $S_1, S_2 \in
%\Real^n$ is defined as 
%\[ 
%S_1 \cap S_2 \rmdef \set{\pp \::\: \pp \in S_1 \text{ and } \pp \in S_2}.
%\] 
%Intersection of two convex polytopes is a convex polytope, while the union of
%two convex polytope is not necessarily a convex polytope. 


\noindent{\bf Constraints.}
% Predicates, Linear Constraints, Rectangular Constraints, and Diagonal 
Let us fix a set $X$ of real-valued variables. 
Before we formally introduce a hybrid automaton we need to define various
constraints on the valuations over $X$ that can be used to specify some of its
components.   

The \emph{predicates} are the most general form of constraints and 
a predicate over $X$ is simply defined as a subset of $\Real^{|X|}$. 
For efficient computer-readable representation of predicates we often define
them using non-linear algebraic equations involving $X$. 
An example of a predicate over the set $\set{\ddot{\theta}, \theta}$  is
$\ddot{\theta} + (g/\ell)\sin(\theta) = 0$ characterizing the motion of an
idealized pendulum (Figure~\ref{pendulum})  where $\theta$ is the angle the
pendulum forms with its rest position, $\ddot{\theta}$ is second derivative of
$\theta$, $g$ is the gravitational constant, while $\ell$ is the length of the
pendulum. 
We write $\pred(X)$ for the set of predicates over $X$.
For a predicate $\pi \in \pred(X)$ we write $\sem{\pi}$ for the set of 
valuations in $\Real^{|X|}$ satisfying the equation $\pi$. 
We write $\top$ for the predicate that is true for all valuations, while $\bot$
for the predicate which is false for all the valuations. 

We say that a predicate $P$ is \emph{polyhedral} if it is defined as the conjunction
of a finite set of linear constraints of the form 
$ a_1 x_1 + \dots + a_n x_n \sim k$, where $k \in \Int$, for all $1 \leq i \leq
n$ we have that $a_i \in \Real, x_i \in X$, and $\sim \in \{<,\leq, =, >,
\geq\}$.  
An example of a polyhedral predicate over the set $\set{x, y, x}$ is
$2x+3y-9z\leq 5$.
We define an \emph{octagonal} predicate as the conjunction of a
finite set of linear constraints over $X$ of the form $x - y \sim k \text{ or }
x \sim k$, where $k \in \Real$, $x, y \in X$, and $\sim \in \{<,\leq, =, >, \geq\}$.
Similarly a \emph{rectangular} predicate is defined as the conjunction of a
finite set of linear constraints over $X$ of the form $x \sim k$, where $\sim
\in \{<,\leq, =, >, \geq\}$, $k \in \Real$, and $x \in X$.
Finally, a \emph{singular} predicate characterizes a \emph{singleton} set and it
can be defined as the set of constraints specifying a fixed value for each
variable, i.e. $x_i {=} k_i$ for $x_i {\in} X$ and $k_i {\in} \Real$.  
We write $\poly(X)$, $\oct(X)$, $\rect(X)$, and $\sing(X)$ for the set of
polyhedral, octagonal, rectangular, and singular predicates, resp., over the set $X$.


\subsection{State Transition Systems}
\label{sts}
\begin{definition}[State Transition System]
  A (labeled) state transition system is a tuple $\Tt = (S, S_0, \Sigma, \Delta,
  AP, L)$ where:  
  \begin{itemize}
  \item $S$ is a (potentially infinite) set of \emph{states}; 
  \item $S_0 \subseteq S$ is the set of \emph{initial states};
  \item $\Sigma$ is a (potentially infinite) set of \emph{actions};
  \item $\Delta \subseteq S \times \Sigma \times S$ is the \emph{transition
      relation}.  
  \item $AP$ is a finite set of \emph{atomic propositions};
  \item $L: S \rightarrow 2^{AP}$ labels every state with a subset of $AP$.
  \end{itemize}
\end{definition}

We say that $\Tt$ is finite (countable), if the sets $S$ and $\Sigma$ are finite
(countable). 
For $s, s' \in S$ and $a \in A$ we write $s{\xrightarrow{a}} s'$ to denote that 
$(s, a, s') \in \Delta$. 
For a state $s \in S$ and action $a \in A$ we define the functions 
$\post, \pre: S \times \Sigma \to 2^S$ as:
\begin{eqnarray*}
\post(s, a) &\rmdef&   \set{s' \::\: s {\xrightarrow{a}} s'} \text{ and }\\
\pre(s, a) &\rmdef&   \set{s' \::\: s' {\xrightarrow{a}} s}.
\end{eqnarray*}


A \emph{run} or a \emph{trajectory} of a state transition system $\Tt$ is a
sequence $\seq{s_0, a_1, s_1, s_2, s_2, \ldots, s_n}$ such that  $s_0 \in S_0$
and for all $0 \leq i < n$ we have that $s_i {\xrightarrow{a_{i+1}} s_{i+1}}$.  
Given an action $a \in \Sigma$ and a state $s$ we write $\post(s,a)$ for the set
of states that have a reachable from $s$ i.e. $\post(s, a) = \set{s' \mid
  (s,a,s') \in \Delta}$.  
$Post(s)=\bigcup_{a \in \Sigma} Post(s,a)$. 
We write $\RUNS(T)$ for the set of all runs of $T$ starting from some initial state.
Denote by $RUNS(T,s_j)$ the runs starting from a state $s_j$. 
For a run $r \in \RUNS(T)$ we define $\LAST(r)$ as the last state of the run
$r$. Given a run $r=s_0, a_1, s_1, s_2, s_2, \ldots, s_n \dots$,
the sequence $L(s_0)L(s_1)L(s_2) \dots L(s_n)\dots$ is called a trace. 
$Trace(T)=\{Trace(r) \mid$ $r$ is a run of $T\}$. 
Given a state $s_j$,  we define 
$Lan(s_j)=\{a_{j+1}a_{j+2}\dots a_n \mid s_j, a_{j+1}, s_{j+1}, a_{j+2}, s_{j+2}, \ldots, a_n, s_n \in RUNS(T,s_j)\}$.

%%%%%%%%%%added today june 19, 2013%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Transition systems are useful for modelling software/hardware systems at various levels 
of abstraction. If the level of abstraction is low, then the transition system 
has a lot of implementation details; on the other  hand, if the level of abstraction is high, then 
there will be fewer implementation details. Consider a piece of software that models
a remote control system which controls three race cars $C_1, C_2, C_3$. 
Before reaching the finish line, a bridge has to be crossed. The bridge can carry exactly one car 
at any point of time, an overload may cause a bridge collapse. 
Assume that we use 3 boolean variables $x,y,z$ to denote the cars that  
are currently on the bridge.  A safety requirement to be enforced is that atmost one of $x,y,z$ can be 1. 
A low level abstraction $L$ can model the situation that from any of the states $x=1, y=0,z=0$
$x=0,y=1,z=0$ or $x=y=0,z=1$, the finish line can be reached. A higher level of abstraction 
$H$ can simply say that the finish line can be reached whenever $x \wedge y \wedge z=0$. $L$ can be obtained 
by refining $H$; that is, by adding more implementation details. Similarly, $H$ can be obtained 
from $L$ by hiding a few implementation details. 

Implementation relations are used for comparing two models of the same system. Consider a transition system $TS$ 
that is an abstraction of some system specification, and a more detailed transition system $TS'$. Implementation relations 
provides techniques to abstract away  details that are irrelevant for the analysis of a given property $P$. This 
can be used to obtain  a smaller model $TS$ from a very large model $TS'$, provided the abstraction preserves 
the property $P$. In this case, checking $TS \models P$ is sufficient to check 
if $TS' \models P$. 

Bisimulation equivalence is an important implementation relation that has been studied in the literature. 
A transition system $TS'$ can simulate a transition system $TS$ if every step of $TS$ can be matched by one 
or more steps of $TS'$. Bisimulation equivalence denotes the possibility of mutual, stepwise simulation. 
Given two transition systems $TS_1$ and $TS_2$, with $TS_i=(S_i, S_{0i}, \Sigma_i, \Delta_i, AP, L_i)$, $i=1,2$,
 a bisimulation relation for $(TS_1, TS_2)$ is a binary relation ${\mathcal R} \subseteq S_1 \times S_2$ such that 
\begin{itemize}
 \item(A) $\forall s \in S_{01}, \exists s' \in S_{02}$ such that $(s,s') \in {\mathcal R}$, and 
 $\forall s' \in S_{02}, \exists s \in S_{01}$ such that $(s',s) \in {\mathcal R}$;
 \item(B) for all $(s_1, s_2) \in {\mathcal R}$, the following is true:
 \begin{itemize}
 \item(1) $L_1(s_1)=L_2(s_2)$,
 \item(2) If $s'_1 \in Post(s_1)$, $\exists s'_2 \in Post(s_2)$ with $(s'_1, s'_2) \in {\mathcal R}$, and 
 \item(3) If $s'_2 \in Post(s_2)$, $\exists s'_1 \in Post(s_1)$ with $(s'_1, s'_2) \in {\mathcal R}$ 
\end{itemize}
\end{itemize}
$TS_1$ and $TS_2$ are bisimulation equivalent denoted $TS_1 \sim TS_2$ if there exists a bisimulation 
relation ${\mathcal R}$ for $(TS_1,TS_2)$.
Consition (A) says that every initial state of $TS_1$ is related to some initial state of $TS_2$, and vice-versa. 
Condition (B.1) says that $s_1, s_2$ are labeled in the same way. This is some form of ``local equivalence''. 
Condition (B.2) says that every outgoing transition of $s_1$ must be matched with some outgoing transition 
of $s_2$; (B.3) says the reverse.  

\input{bisim1.tex}

Figure \ref{bisim1} gives two transition systems which are not bisimilar. 
The transition systems in figure \ref{bisim1} model the flights of two airlines. It is clear that 
for the first airline, it is possible to reach Shimla as well as Delhi from Mumbai; 
the airline on the right however, has exactly one choice of destination from Mumbai. 

\begin{lemma}
\label{trace-eq}
 $TS_1 \sim TS_2$ implies $Trace(TS_1)=Trace(TS_2)$.
\end{lemma}


Bisimulation is defined in terms of the direct successors of a state. This can be extended to (finite or infinite) paths:
\begin{lemma}
\label{bisim-path}
Let $TS_1, TS_2$ be two transition systems over a set of propositions $AP$, and let ${\mathcal R}$ be a 
bisimulation relation for $(TS_1, TS_2)$. Then, for each finite or infinite run $s_0 s_1 s_2 \dots$ of $TS_1$, 
there exists a run $s'_0 s'_1 s'_2 \dots$ of $TS_2$ of the same length such that 
$(s_i, s'_i) \in {\mathcal R}$ for all $i \geq 0$. 
\end{lemma}

{\it Model Checking} proposed by Ed Clarke, J. Sifakis and A. Emerson is a very widely 
used automated technique that, given a finite state model of a system, and a property, 
systematically checks whether this property holds for a given state in that model. 
The three main steps in a model checking procedure are (i) modelling the system 
under consideration : this means abstracting unnecessary details from the system and coming up 
with an appropriate finite size model, (ii) writing the properties to be checked formally : this can be done 
using some suitable property specification language, and (iii) analyze the model with respect to the 
property. If the property is satisfied, we can  move on; otherwise, 
a counter example (run that violates the property) will be obtained. 
We can analyze this counter example, and if needed, refine the model and/or the property and 
repeat the entire procedure.

State transition systems given in section \ref{sts} are a fundamental model 
for modeling software and hardware systems. Transition systems serve as 
models for concurrent systems, petri nets, state charts, sequence charts; 
they are also used as unfoldings of program graphs. Temporal logics 
introduced by Amir Pnueli, is one of the foremost property specification languages 
used in computer science. 
Temporal logics extend propositional or predicate logics by modalities 
that are useful to capture the change of behaviour of a system over time. 
The elementary temporal modalities involved are 
$\Diamond$ (which stands for ``eventually'') and $\Box$ (which stands for 
``now and forever''). 

{\it Linear Temporal Logic (LTL)} is a temporal logic widely used in property specification. 
Given a set $AP$ of atomic propositions, the syntax of LTL is as follows: 
$$\varphi::==true|a|\varphi_1 \wedge \varphi_2|\neg \varphi|\varphi_1 \until \varphi_2$$
where $a \in AP$. $\varphi_1 \until \varphi_2$ means that property $\varphi_1$  keeps on holding 
until property $\varphi_2$ is true. It must be noted that 
$\Diamond \varphi \equiv true \until \varphi$ and $\Box \varphi=\neg \Diamond \neg \varphi$. LTL formulae are 
interpreted over transition systems. For a run $r=s_0s_1s_2 \dots $ of 
the transition system, let $\sigma=Trace(r)$. Denote by $\sigma[j]$ the 
trace starting from $s_j$. Then the satisfaction of LTL formulae is defined as follows:
\begin{eqnarray*}
 &&\sigma \models a~\mbox{iff}~a \in L(s_0)\\
 &&\sigma \models \varphi_1 \wedge \varphi_2~\mbox{iff}~\sigma \models \varphi_1~\mbox{and}~\sigma \models \varphi_2\\
 &&\sigma \models \varphi ~\mbox{iff}~\sigma \nvDash \varphi\\
 &&\sigma \models \varphi_1 \until \varphi_2~ \mbox{iff there exists}~j \geq 0,~\sigma[j] \models \varphi_2~\mbox{and for}\\
 &&~~~~~~~~~~~~~~~~~~\mbox{all}~0 \leq i < j,~\sigma[i]\models \varphi_1
 \end{eqnarray*}

Consider the  transition system $TS$ 
in Figure \ref{ts1} and the LTL formula $\varphi=d \until (c \wedge \neg d)$. 
Does $TS \models \varphi$ (read as $\varphi$ holds in $TS$)? 
This is true iff all runs of $TS$ satisfy $\varphi$. It is clear that 
$TS \nvDash \varphi$ since the run $r$ with $Trace(r)=\{c\}\{c,d\}\{c,d\}$ does not satisfy 
$\varphi$.

\input{ts1}

Given a finite state transition system $TS$ over a set of atomic propositions $AP$, and 
a property specification written in LTL over a set $AP' \subseteq AP$ of atomic propositions, 
the model checking question amounts to asking ``does $TS \models \varphi$''? There are various tools 
that do LTL model checking. SPIN, developed by Holzmann, is one of the most well known LTL model checkers. 
In SPIN, transition systems are described in a modelling language called Promela, and 
LTL formulae are checked using the algorithm given by Gerth et al \cite{gerth}. 
Another popular property specification language is {\it Computation Tree Logic (CTL)}. 
One of the most well known CTL model checkers is NuSMV, developed by Cimmatti et al. 
NuSMV also supports LTL model checking.  


The reachability problem is another key verification problem for state transition
systems. Given a state transition system $TS$ and a set of
target states $F$, the reachability problem asks whether there is a
run $r \in \RUNS(T)$ such that $\LAST(r) \in F$.  
For finite state transition systems the reachability problem can be solved by
using classical depth-first search (DFS) or breadth-first search (BFS)
algorithms for graph traversal. 
The complexity of BFS algorithms is $O(|S|+|\Delta|)$.
SPIN and NuSMV provide efficient algorithms to solve
reachability problem for finite state transition systems.
For large finite state transition systems it is often not possible to store the
transition system explicitly.
There are efficient data-structures like reduced-ordered \emph{binary decision
  diagrams} that allow symbolic representation of states sets and transition
relations as Boolean functions, and efficient operations like union,
intersection, complementation, emptiness checking, and existential
quantification of symbolically represented state sets.
Verification tool NuSMV implements symbolic representation of state transition
systems and symbolic reachability analysis of these systems.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\input{q1}
\input{q2}
Bisimulation, as defined above is useful in comparing two state transition systems. 
Al alternative perspective is to consider bisimulation as a relation between 
the states of a single state transition system. 
Defining this relation appropriately helps in reducing the size 
of the state transition system, which comes in very handy for efficient model checking. 

Let $TS=(S, S_0, \Sigma, \Delta, AP, L)$ be a finite state transition system. 
A bisimulation for $TS$ is a binary relation ${\mathcal R}$ on $S$ such that 
for all $(s_1, s_2) \in {\mathcal R}$,
\begin{itemize}
 \item $L(s_1)=L(s_2)$,
 \item If $s'_1 \in Post(s_1)$, then there exists an $s'_2 \in Post(s_2)$ such that $(s'_1, s'_2) \in {\mathcal R}$,
 \item If $s'_2 \in Post(s_2)$, then there exists an $s'_1 \in Post(s_1)$ such that $(s'_1, s'_2) \in {\mathcal R}$.
\end{itemize}
We say that states $s_1, s_2$ are bisimulation equivalent denoted $s_1 \sim_{TS} s_2$ if there exists a bisimulation 
relation ${\mathcal R}$ for $TS$ with $(s_1,s_2) \in {\mathcal R}$.
Given $TS$, we use the bisimulation relation $\sim_{TS}$ for minimizing the state space of $TS$. 
The quotient transition system $TS/\sim$ is defined 
by  
$$TS/\sim=(S/\sim, S'_0, \{\tau\}, \Delta', AP, L')$$ where 
\begin{itemize}
 \item $S'_0=\{[s]_{\sim} \mid s \in S_0\}$,
 \item $\Delta'=\{([s]_{\sim}, \tau, [s']_{\sim}) \mid (s,\alpha,s') \in \Delta\}$,
 \item $L'([s]_{\sim})=L(s)$
 \end{itemize}
$TS/\sim$ is called the bisimulation quotient of $TS$. The state space of 
$TS/\sim$ is teh quotient space of $TS$ : the initial states 
in $TS/\sim$ are the $\sim$-equivalence classes of the initial states 
of $TS$; each transition $(s,a,s') \in \Delta$ induces 
a transition from $[s]_{\sim}$ to $[s']_{\sim}$. 
The action is irrelevant, and hence, we keep a unique action $\tau$. 
The state labeling $L'$ is well defined, since 
all states in $[s]_{\sim}$ are labeled same, by definition of bisimulation. 
Note that for model checking purposes, we only need the traces 
of the transition system; the actions play no role. 



We now give an example to see the state space reductions possible by quotienting. 
Consider the situation at an airport with $n$ aircrafts at bay. 
Each aircraft is one of the two states : ready for take-off or 
not ready for take-off. Modeling this as a transition system $TS$, 
with $S=\{(a_1,a_2, \dots, a_n) \mid a_i \in \{0,1\}\}$, 
we have states corresponding to all $n$-tuples
of possibilities of aircraft $i$ being ready for take-off or not. 
However, intuitively, $L(s)$ denotes the number of aircrafts 
that are ready for take-off at any point of time. 
Figures \ref{q1}, \ref{q2} shows the system before and after quotienting for the case 
of $n=3$. 


==> oldverification.tex <==
Formal modeling and verification of systems is the set of techniques that employ
rigorous mathematical reasoning to analyze properties of a system. 
In this article we concentrate on model checking---a formal verification
framework introduced by Clarke, Sifakis and Emerson~\cite{CES09}---that, given a
formal description of a system and its specification, systematically
verifies whether the specification holds for the system model.  
Since, by definition the states of a dynamical system changes with time,
classical propositional logic is not sufficient to reason with temporal
properties of such dynamical systems.
Temporal logics extend propositional or predicate logics by modalities 
that are useful to capture the change of behaviour of a system over time. 
Manna and Pnueli~\cite{MP92,TM0} were the first one to propose and promote the
use of temporal logic to specify properties of dynamical systems in the context
of system verification.
\emph{Linear temporal logic} (LTL)~\cite{MP92}, \emph{computation tree logic}
(CTL) and its generalization CTL$^*$~\cite{MP92,CGP99}, and modal
$\mu$-calculus~\cite{Eme96} are some of the popular temporal logics used for the
system specification. 
Timed and weighted extensions of these logics  e.g. metric temporal logics
(MTL and MITL~\cite{OW08}), duration calculus (DC)~\cite{GNRR93}, and 
weighted logics~\cite{BBR04,Bou06} have also been proposed to specify more
involved quantitative properties of hybrid dynamical systems.

In this article we limit the discussion to simple qualitative properties of
hybrid systems that broadly can be classified into the following two broad
categories: 
\begin{itemize}
\item 
  \emph{reachability properties} that ask whether the system can reach a
  configuration satisfying certain property $p$? 
  (symbolically, we write $\Diamond p$ and we say \emph{eventually} $p$),
  and 
\item 
  \emph{safety properties} that ask whether the system can stay forever in
  configurations satisfying certain property $p$? 
  (symbolically, we write $\Box p$ and we say \emph{globally} $p$).   
\end{itemize}
The linear temporal logic, LTL, provides a formal language to specify more
involved nesting of such properties with ease.  
We begin this section (Section~\ref{sec:LTL}) by introducing Kripke structures
that provide a way to mark states of the hybrid automata with properties of
interest, and present the syntax and semantics of LTL that are interpreted over
Kripke structures. 
In Section~\ref{sec:undec} we formally introduce LTL model-checking problem for
hybrid automata, and show that in general this problem is undecidable.
Finally, in Section~\ref{sec:finiteBisum} we introduce the notion of
bisimulation, and show that the existence of a finite bisimulation implies the
decidability of LTL model-checking problem.

\subsection{Hybrid Kripke Structures and Linear Temporal Logic}
\label{sec:LTL}
The formal specification of the underlying system begins by identifying key
properties of interests (called atomic propositions) regarding the states of the
system under verification.  
Kripke structures provide a way to label the states of state-transition graphs
with such atomic propositions, and the linear temporal logic specifies
properties of the sequence of the truth values of these propositions, called the
\emph{traces}, for the runs of corresponding transition system.

\begin{definition}[Kripke Structure]
  A \emph{Kripke Structure} is a tuple $\Kk = (\Tt, P, L)$ where:
  \begin{itemize}
  \item 
    $\Tt = (S, S_0, \Sigma, \Delta)$ is a state transition graph, 
  \item 
    $P$ is a finite set of \emph{atomic propositions}, and 
  \item 
    $L: S \rightarrow 2^{P}$ is a labeling function that labels every state
    with a subset of $P$. 
  \end{itemize}
\end{definition}

\begin{definition}[Hybrid Kripke Structure]
  A \emph{Hybrid Kripke Structure} is a tuple $\Kk = (\Hh, P, L)$ where:
  \begin{itemize}
  \item 
    $\Hh = (M, M_0, \Sigma, X, \Delta, I, F, V_0)$ is a hybrid automaton,
  \item 
    $P$ is a finite set of \emph{atomic propositions}, and 
  \item 
    $L: M \rightarrow 2^{P}$ is a labeling function that labels every mode
    with a subset of $P$. 
  \end{itemize}
\end{definition}
The semantics of a hybrid Kripke structure is given by an infinite state transition system.  
Given an action $a \in \Sigma$ and a state $s$ we write $\post(s,a)$ for the set
of states that are  reachable from $s$ on $a$ i.e. $\post(s, a) = \set{s' \mid
  (s,a,s') \in \Delta}$.  $\post(s)=\bigcup_{a \in \Sigma} \post(s,a)$. 
We write $\RUNS(T)$ for the set of all runs of $T$ starting from some initial state.
Denote by $\RUNS(T,s_j)$ the runs starting from a state $s_j$. 
For a run $r \in \RUNS(T)$ we define $\LAST(r)$ as the last state of the run
$r$. Given a run $r=s_0, a_1, s_1, s_2, s_2, \ldots, s_n \dots$,
the sequence $L(s_0)L(s_1)L(s_2) \dots L(s_n)\dots$ is called a trace. 
$\Trace(T)=\{\Trace(r) \mid$ $r$ is a run of $T\}$. 
Given a state $s_j$,  we define 
$Lan(s_j)=\{a_{j+1}a_{j+2}\dots a_n \mid s_j, a_{j+1}, s_{j+1}, a_{j+2}, s_{j+2}, \ldots, a_n, s_n \in \RUNS(T,s_j)\}$.
The set of all traces is given by $Lan(\Kk)=\bigcup_{s \in M_0}Lan(s)$.  


\noindent {\it Linear Temporal Logic (LTL)} is a temporal logic widely used in property specification. 
Given a set $AP$ of atomic propositions, the syntax of LTL is as follows: 
$$\varphi::==true|a(\in AP)|\varphi_1 \wedge \varphi_2|\neg \varphi|\varphi_1 \until \varphi_2$$
LTL formulae are 
interpreted over kripke structures. For a run $r=s_0s_1s_2 \dots $ of 
the kripke structure, let $\sigma=Trace(r)$. Denote by $\sigma[j]$ the 
trace starting from $s_j$. Then the satisfaction of LTL formulae is defined as follows:
\begin{eqnarray*}
 &&\sigma \models a~\mbox{iff}~a \in L(s_0)\\
 &&\sigma \models \varphi_1 \wedge \varphi_2~\mbox{iff}~\sigma \models \varphi_1~\mbox{and}~\sigma \models \varphi_2\\
 &&\sigma \models \varphi ~\mbox{iff}~\sigma \nvDash \varphi\\
 &&\sigma \models \varphi_1 \until \varphi_2~ \mbox{iff there exists}~j > 0,~\sigma[j] \models \varphi_2~\mbox{and for}\\
 &&~~~~~~~~~~~~~~~~~~\mbox{all}~0 \leq i < j,~\sigma[i]\models \varphi_1
 \end{eqnarray*}
 Given a trace $\sigma$ and an LTL formula $\varphi$, we say that $\sigma \models \varphi$ 
 iff $\sigma[0] \models \varphi$. Also, $L(\varphi)=\{\sigma \mid \sigma[0] \models \varphi\}$.
 Note that $\Diamond \varphi \equiv true \until \varphi$ and $\Box \varphi=\neg \Diamond \neg \varphi$.

\begin{definition}
 Given a system modeled as a Kripke structure $\TS$, and a specification written as an LTL 
 formula $\varphi$, the {\it LTL model checking} question amounts to asking 
 whether $\TS$ satisfies $\varphi$. This is denoted $\TS \models \varphi$. 
 We say that $\TS \models \varphi$ iff 
 $Lan(\TS) \subseteq L(\varphi)$.
\end{definition}

\input{inc-1}

Consider the kripke structure $\TS$ 
in Figure \ref{ts1} and the LTL formula $\varphi=d \until (c \wedge \neg d)$. 
$\TS \nvDash \varphi$ since the run $r$ with $\Trace(r)=\{c\}\{c,d\}\{c,d\}$ does not satisfy 
$\varphi$.

\input{ts1}
 For a kripke structure $\TS$, we are interested in checking three kinds of LTL properties: 
(i) reachability, (ii) safety and (iii) liveness. Reachability 
 is the simplest kind of property that we can check on a structure : 
it checks if a chosen bad state is reachable from some initial state. A bad state 
typically represents a situation violating some specification, 
thus, reachability of a bad state amounts to the violation 
of some specification. Safety guarantees that a bad state will never be reached; 
thus, the structure under consideration is ``safe''. Checking safety properties 
amounts to checking that all runs of the structure do not encounter the bad state. 
Note however that safety properties cannot be used to check progress requirements; a structure 
doing nothing will be safe, since it never enters a bad state. For checking progress requirements, we 
use liveness properties. Liveness checks that the structure is ``live'' : it guarantees 
the recurrence of a ``good state''.  Model checking safety critical systems  involves 
writing properties which combine checking for reachability, safety and liveness.  

\begin{example}
\label{lift}
As an example, let us see how to write specifications in LTL 
for an elevator operating across $k$ floors.
%as follows: The states of ${\mathcal H}$ are $f_0,f_1,f_2, \dots, f_k$ 
%representing floors 0 to $k$.  A variable $x$ measures the speed with which the elevator moves between any two floors 
%$i$ and $j$.  Let $\dot{x} \in [1,5]$ denote the 
%rate at which the elevator moves up/down between any two floors. 
%At any floor, the door of the lift closes in less than one time unit 
%from the time of opening. Any edge that takes the lift between 
%floors $i,j$ has the guard $x=|j-i|?x'=0$. 
%Figure \ref{lift} gives the hybrid kripke structure ${\mathcal H}$ for floors 0,1. 
Let $op_i, fl_i$ and $req_i$ be atomic propositions representing 
``the door at floor $i$ is open'', `` the lift is at floor $i$ and is not moving'' and 
``there is a request for the lift to move to the $i$th floor'' respectively. 
%the initial state of ${\mathcal H}$ corresponds to the lift waiting 
%at floor 0. 
The following are some specifications in English and their LTL counterparts:
\begin{enumerate}
\item Reachability property : {\it The lift will visit the ground floor  sometime}. $\varphi_1=\Diamond floor_0$.
 \item Safety property : {\it The door of the lift is never open at a floor
if the lift is not present there}. $\varphi_2=\Box[\bigwedge_{i=0}^k(\neg fl_i \Rightarrow \neg op_i)]$. 
\item Liveness property : {\it The lift keeps coming back to the ground floor}.
$\varphi_3=\Box[\neg fl_0 \Rightarrow \Diamond fl_0] \wedge \Box \Diamond fl_0$. 
\item Combining safety and liveness : 
{\it A requested floor will be served sometime}. $\varphi_4=\Box[\bigwedge_{i=0}^k (req_i \Rightarrow \Diamond fl_i)]$.
\end{enumerate}
\end{example}

 
There are various tools that do LTL model checking. SPIN, developed by Holzmann, is one of the most well known LTL model checkers. 
In SPIN, transition systems are described in a modelling language called Promela, and 
LTL formulae are checked using the algorithm given by Gerth et al \cite{GPVW95}.

%\subsection{Model Checking for Hybrid Automata}
%\label{efficientFV}

\subsection{Undecidability of LTL Model Checking}
\label{sec:undec}
In this section, we show that, in general, LTL model checking of hybrid kripke structures is undecidable.
The proof  uses
reductions from the halting problem of two-counter \emph{Minsky
  machines}~\cite{Min67}. 

A Minsky machine $\Aa$ is a tuple $(L, C)$ where:
${L = \set{\ell_0, \ell_1, \ldots, \ell_n}}$ is the set of
instructions. There is a distinguished terminal instruction  $\ell_n$ called $HALT$.
${C = \set{c_1, c_2}}$ is the set of two \emph{counters};
the instructions $L$ are of the following types:
\begin{enumerate}
\item (increment $c$) $\ell_i : c := c+1$;  goto  $\ell_k$,
\item (test-and-decrement $c$) $\ell_i$ : if $(c >0)$ then
  $(c:= c - 1;$ goto $\ell_k)$ else goto $\ell_m$,
  \item (Halt) $\ell_n: HALT$.
\end{enumerate}
where $c \in C$, $\ell_i, \ell_k, \ell_m \in L$.

A configuration of a Minsky machine is a tuple $(\ell, c, d)$ where
$\ell \in L$ is an instruction, and $c, d$ are natural numbers that specify the value
of counters $c_1$ and $c_2$, respectively.
The initial configuration is $(\ell_0, 0, 0)$.
A run of a Minsky machine is a (finite or infinite) sequence of
configurations $\seq{k_0, k_1, \ldots}$ where $k_0$ is the initial
configuration, and the relation between subsequent configurations is
governed by transitions between respective instructions.
The run is a finite sequence if and only if the last configuration is
the terminal instruction $\ell_n$.
Note that a Minsky machine has exactly one run starting from the initial
configuration. 
The \emph{halting problem} for a Minsky machine asks whether 
its unique run ends at the terminal instruction $\ell_n$.
It is well known~(\cite{Min67}) that the halting problem for
two-counter Minsky machines is undecidable.



\begin{theorem}
\label{undec}
LTL model-checking problem for hybrid kripke structures is undecidable.
\end{theorem}
\begin{proof}
Given a two counter machine ${\cal A}$, we construct a hybrid kripke structure ${\cal H}$ and an LTL formula 
$\varphi$ such that ${\cal H}\models \varphi$ iff ${\cal A}$ halts. The modes of 
${\cal H}$ are labeled with the labels $l_i$ of instructions. There is a unique mode of ${\cal H}$ labeled $HALT$ 
which corresponds to the terminal instruction of $\Aa$. The increment, decrement and test 
instructions are encoded by suitable modules in ${\cal H}$. 
The variables of ${\cal H}$ are $X=\{x_1,x_2,y,z,z_1\}$ with $m(x_1)=m(x_2)=m(y)=m(z)=1$ and $m(z_1)=2$ for all modes $m$. 
The initial mode is labeled by $l_0$, the label of the first instruction. 
We illustrate here the case of the increment instruction $l_i$ : increment $c$ and goto $l_j$. 

The values of the counters $c,d$ are encoded as $x_1=\frac{1}{2^c}$ and $x_2=\frac{1}{2^d}$.
After the execution of each instruction, $x_1, x_2$ will contain the current values of counters $c,d$ 
encoded in the above form. For instance, if we have $x_1=\frac{1}{2^c}$, $x_2=\frac{1}{2^d}$ before 
incrementing counter $c$, then at the end of simulating the increment instruction, we will have 
$x_1=\frac{1}{2^{c+1}}$ and $x_2=\frac{1}{2^d}$.

Mode $l_i$ is entered with $y=0$, $x_1=\frac{1}{2^c}$ and $x_2=\frac{1}{2^d}$. On entering mode $A$, 
we have $x_1=1, y= 1-\frac{1}{2^c}, x_2=\frac{1}{2^d}+(1-\frac{1}{2^c})$  or $x_2=1-\frac{1}{2^c}-\eta$
if $\frac{1}{2^d}+\eta=1$, $\eta \leq 1-\frac{1}{2^c}$ and $z=0$.
Mode $B$ can be entered if $x_2,y<1$ and $x_1 > 1$. Assume $k>0$ units of time was spent at mode $A$.
 This gives $y=1-\frac{1}{2^c}+k, x_2=\frac{1}{2^d}+(1-\frac{1}{2^c})+k$ (or $1-\frac{1}{2^c}-\eta+k$,
 or $1-\eta'$ if $1-\frac{1}{2^c}-\eta+\eta'=1$, $\eta' \leq k$), $z=k$, $x_1=0,z_1=0$ 
 on entering mode $B$. We can reach mode $l_j$ only if the values of $z$ and $z_1$ are the same.
 Assume $l$ units of time was spent at $B$. Then $z=k+l, z_1=2l$, 
 $x_2=\frac{1}{2^d}+(1-\frac{1}{2^c})+k+l,x_1=l,y=1-\frac{1}{2^c}+k+l$.
  To satisfy the constraints $z=z_1,y=1$,  we have $k=l$ and $k+l=2k=\frac{1}{2^c}$ giving 
 $x_1=\frac{1}{2^{c+1}}, x_2=\frac{1}{2^d}$,$y=0$ at $l_j$. 
 
 
In a similar way, we can encode decrement instructions and zero test instructions. 
The LTL formula $\varphi=l_0 \wedge \Diamond HALT$ will be satisfied by 
${\cal H}$ iff $\Aa$ halts. This shows that LTL model checking of 
hybrid kripke structures is undecidable.
   
\end{proof}


\subsection{Finite Bisimulation and Decidability} 
\label{sec:finiteBisum}
\label{bisim}
\input{finiteBisimulation}


==> prelims.tex <==
%\subsection{Notation}
%\input{constraints}

\section*{Notation}
Let $\Real$ be the set of real numbers, $\Rplus$ be the set of non-negative
real numbers, and $\Int$ be the set of integers. 
%{\bf Valuations, Points, and Vectors.} 
Let $X$ be a set of real-valued variables. 
A \emph{valuation} on $X$ is a function $\nu : X {\to} \Real$ and we write $V(X)$
for the set of valuations on $X$.
If $|X| = n$ then, abusing notation, we also treat a valuation $\nu$ as a point in
$\Real^n$ that is equipped with the standard \emph{Euclidean norm}
$\norm{\cdot}$. 
%We denote points (valuations) in this valuation space by $\pp, \pq$ and  vectors
%by $\vr, \vv$.
%We denote the $i$-th coordinate of point $\pp$ and vector $\vr$ by
%$\pp(i)$ and $\vr(i)$, respectively.
%Similarly, for a variable $x \in X$ we denote the coordinate of point $\pp$ and
%vector $\vr$ corresponding to $x$ by $\pp(x)$ and $\vr(x)$, respectively.
%We write $\vzero$ for a vector with all its coordinates equal to $0$; 
%its dimension is often clear from the context.
%The distance $\norm{\pp, \pq}$ between points $\pp$ and $\pq$ is defined as
%$\norm{\pp - \pq}$. 
%For two vectors ${\vv_1, \vv_2 \in \Real^n}$, we write $\vv_1 \dotprod \vv_2$
%to denote their dot product defined as $\sum_{i=1}^n \vv_1(i)\cdot\vv_2(i)$.
%
%
%\noindent{\bf Boundedness and Interior.} 
%We denote a {\em closed ball} of radius $d \in \Rplus$ centered at $\pp$ as
%$\ball{d}{\pp} {=} \set{\pq {\in} \Real^n \::\: \norm{\pp,\pq} \leq d}$.
%We say that a set $S \subseteq \Real^n$ is {\em bounded} if there exists
%$d \in \Rplus$ such that for all $\pp, \pq \in S$ we have
%$\norm{\pp,\pq} \leq d$.
%The {\em interior} of a set $S$, $\interior(S)$, is the set of all points
%$\pp \in S$ for which there exists $d > 0$ s.t. $\ball{d}{\pp} \subseteq S$.
%
%
%\noindent{\bf Convexity.} A point $\pp$ is a \emph{convex
%  combination} of a finite set of points $P = \set{\pp_1, \pp_2, \ldots, \pp_k}$ if
%there are $\lambda_1, \lambda_2, \ldots, \lambda_k \in [0, 1]$ such that
%$\sum_{i=1}^{k} \lambda_i = 1$ and $\pp = \sum_{i=1}^k \lambda_i \cdot \pp_i$.
%The \emph{convex hull} $\CVH{S}$ of a set $S$ is then the set of all points
%that are convex combinations of points in $S$.
%We say that $S \subseteq \Real^n$ is {\em convex} iff for all
%$\pp, \pq \in S$ and all $\lambda \in [0,1]$ we have
%$\lambda \pp + (1-\lambda) \pq \in S$ and moreover,
%$S$ is a {\em convex polytope} if it is bounded and there exists $k \in \Nat$, a
%matrix $A$ of  size $k \times n$ and a vector $\vb \in \Real^k$ such that $\pp
%\in S$ iff $A\pp \leq \vb$. 
%We write $\rows{M}$ for the number of rows in a matrix $M$, here $\rows{A}=k$. 
%Convex polytopes can also be represented using the notion of a vertex.
%A point $\pp$ is a \emph{vertex} of a convex polytope $P$ if it is
%not a convex combination of two distinct (other than $\pp$) points in $P$. 
%For a convex polytope $P$ we write $\Vtx{P}$ for the finite set of points that
%correspond to the vertices of $P$.  
%Each point in $P$ can be written as a convex combination of the points in
%$\Vtx{P}$, or in other words, $P$ is the \emph{convex hull} of $\Vtx{P}$. 
%
%\noindent{\bf Constraints.}
%Let us fix a set $X$ of real-valued variables. 
%Before we formally introduce a hybrid automaton we need to define various
%constraints on the valuations over $X$ that can be used to specify some of its
%components.   




==> todos.tex <==




==> undecidability.tex <==
The strongest known decidability for hybrid automata concerns
a class~\cite{PV94} of linear hybrid automata with rectangular inclusions.
These are hybrid automata where 
all the variables are linear, predicates are of the form $x \sim c$,  variable
assignments are reset assignments, and $dif(x,l)$ is a constant function. 
That is,  variable $x_i$ is such that $dif(l,x_i)$ is of the form $\dot{x_i} \in
[L_i, U_i]$ for all $l \in L$. 
In this section, we show that this is indeed, the boundary of decidability. 
Any relaxation of the restrictions by (i)admitting a single variable with non
constant activities, like a two-slope variable or a stopwatch, (ii) admitting
stronger enabling conditions,  like comparing variables, (iii) admitting
variable-to-variable assignments,  (iv) admitting stronger invariants, such as
triangular differential inclusions, lead to undecidability. 
Such an invariant is a predicate of the form $\dot{x} \leq \dot{y}$  
and conjunctions of such inequalities. 
In this section, we sketch the proof of these undecidability results using
reductions from the halting problem of two-counter \emph{Minsky
  machines}~\cite{Min67}. 

A Minsky machine $\Aa$ is a tuple $(L, C, D)$ where:
${L = \set{\ell_0, \ell_1, \ldots, \ell_n}}$ is the set of
states including the distinguished terminal state $\ell_n$;
${C = \set{c_1, c_2}}$ is the set of two \emph{counters};
${D = \set{\delta_0, \delta_1, \ldots, \delta_{n-1}}}$ is the set of
transitions of the following type:
\begin{enumerate}
\item (increment $c$) $\delta_i : c := c+1$;  goto  $\ell_k$,
\item (test-and-decrement $c$) $\delta_i$ : if $(c >0)$ then
  $(c:= c - 1;$ goto $\ell_k)$ else goto $\ell_m$,
\end{enumerate}
where $c \in C$, $\delta_i \in D$ and $\ell_k, \ell_m \in L$.

A configuration of a Minsky machine is a tuple $(\ell, c, d)$ where
$\ell \in L$ is a state, and $c, d$ are natural numbers that specify the value
of counters $c_1$ and $c_2$, respectively.
The initial configuration is $(\ell_0, 0, 0)$.
A run of a Minsky machine is a (finite or infinite) sequence of
configurations $\seq{k_0, k_1, \ldots}$ where $k_0$ is the initial
configuration, and the relation between subsequent configurations is
governed by transitions at their respective states.
The run is a finite sequence if and only if the last configuration is
the terminal state $\ell_n$.
Note that a Minsky machine has exactly one run starting from the initial
configuration. 
The \emph{halting problem} for a Minsky machine asks whether
its unique run is finite.
It is well known~(\cite{Min67}) that the halting problem for
two-counter Minsky machines is undecidable.

 \subsection{Some Simple Gadgets}
In the following gadgets, every edge has a constraint $\bigwedge_{x \in V}(x
\leq 4g(x,l))$, where $g(x,l)$  is the maximum permissible slope of variable $x$
in location $l$.  
To avoid clutter, we do not write these constraints in the figures..
Let $x(e)$ denote the value of variable $x$ 
on traversing edge $e$, before any variable assignments.

 \begin{lemma}(Wrapping Lemma)
 \label{wrap:lem}
Consider the hybrid automaton given in Fig.~\ref{threeinone}(a). 
Assume that when edge $e_1$ is traversed entering $W$, 
$c=\gamma, d=\delta$, where $0 \leq \gamma \leq 2g$ and $0 \leq \delta \leq 2h$. Let 
$dif(c,v)$, $dif(d,v)$ be respectively  $\dot{c}=g$ and $\dot{d}=h$.
Then the next time when edge $e_2$ is traversed out of $W$, $c=\gamma$ and $d=\delta$. 
\end{lemma}
\begin{proof}
 
\input{wrapEqualAssign} 

Assume that while entering $v$, $c=2g-k, d=2h-m$, with $k,m \geq 0$. 
Hence, $c(e_1)=2g-k, d(e_1)=2h-m$.
Exactly 4 units of time will be spent at $v$ before traversing $e_4$. 
Since $c \leq 4g$ is an enabling condition on every edge, we must traverse 
the loop $c=4g?c:=0$ once before traversing $e_2$. 
The time spent $t$ elapsed at  $v$ before taking this loop is 
$t=\frac{1}{g}[4g-c(e_1)]$. 
For $a=4$ to hold, we must elapse $4-t$ time 
at $v$. Hence, when $e_2$ is traversed,
we have $c(e_2)=g[4-(\frac{1}{g}[4g-c(e_1))]=c(e_1)$. Similarly,
it can be shown that $d(e_1)=d(e_2)$.
\end{proof}

\begin{lemma}(Equality Lemma)
\label{eq:lem}
 Consider the hybrid automaton in figure \ref{threeinone}(b). 
 Assume that when edge $e_1$ is traversed into $E$, 
 $c=\gamma, d=\delta$, with $0 \leq \gamma, \delta \leq 2g$.
  Let $dif(c,v)$, $dif(d,v)$ be respectively  $\dot{c}=g$ and $\dot{d}=g$.
  The edge $e_2$ can be traversed iff $\gamma=\delta$. When $e_2$ is traversed,
  $c=d=\gamma$.
\end{lemma}
 \begin{proof}
%\input{equality}
It is easy to see that if $e_2$ is traversed, then $c(e_2)=\gamma$. 
This can be seen from Lemma~\ref{wrap:lem}. 
Assume now that on entering $v$ thrugh $e_1$, $\gamma \neq \delta$. 
Let $\gamma=2g-k, \delta=2g-m$, with $m \neq k$. 
Then it is clear that the loop which resets $c,d$ together cannot be taken,
since $m \neq k$. 
Assume that  $k < m$. 
Then $c$ attains $4g$ faster than $d$, and is reset.
The time elapse  for $c$ to attain $4g$ is  $t=\frac{1}{g}[2+\frac{k}{g}]$.
The value of $d$ when the loop is taken is $2g-m+2g+k=4g-(m-k)$. 
When $d$ attains $4g$, the total time spent at $v$ is 
$t+\frac{1}{g}(m-k)=2+\frac{m}{g}<4$. 
Clearly, when $d$ attains $4g$, the loop cannot be traversed; further, 
to traverse $e_2$, $2-\frac{m}{g}$ time has to be spent in $v$. 
Then $d=4g+(2g-m) > 4g$; in which case, $e_2$ cannot be taken.
Similar arguments hold good when $m < k$.

Thus, $e_2$ can be traversed iff $m=k$ and hence $\gamma=\delta$.
\end{proof}

\begin{lemma}
  \label{assgn:lem}
  Consider the hybrid automaton in Fig.\ref{threeinone}(c).
  Assume that when edge $e_1$ is traversed into $A$, $c=\gamma$, $ 0 \leq \gamma
  \leq 2g$.  
  Let $dif(c,v)$, $dif(d,v)$ be respectively  $\dot{c}=g$ and $\dot{d}=h$. 
  Then the next time when $e_2$ is traversed out of $v$, $c=\gamma,
  d=\frac{h}{g}\gamma$. 
\end{lemma}
\begin{proof}
  The proof is similar to lemmas~\ref{eq:lem} and~\ref{wrap:lem} and hence
  omitted. 
\end{proof}

\begin{theorem}
\label{thm:one}
 For every $g > 0$ with $ g \neq 1$, the reachability problem for hybrid systems with 
 \begin{itemize}
  \item one skewed clock of slope $g$, and any number of clocks,
  \item weak predicates with variable equality tests,
  \item reset assignments
 \end{itemize}
is undecidable.
\end{theorem}
\begin{proof}
 We reduce the halting problem for two counter machines 
 to this problem.  Let $M$ be a two counter machine with counters $m,n$. 
 We use clock variables $c, d$ corresponding to counters $m,n$. Assume 
 that $g=2$. The counter value $m=k$ is encoded as $c=2^{1-k}$; 
 similarly, the counter value $n=j$ is encoded as $d=2^{1-j}$. 
 
 We look at the implementation of the instruction $l_i : Dec(m)$, goto $l_j$. 
 Decrementing $m$ corresponds to doubling $c$, and keeping $d$ unchanged.
  In addition to clocks $c,d$, we use a skewed clock variable $t$ of slope 2.
  An atomic  weak predicate is of the form $x \leq c$ or $x \geq c$. A weak predicate 
  is obtained as a conjunction of atomic weak predicates. An equality test is  
  of the form $x=y$ for variables $x,y$.
\input{doublingSkew}
When we come out of $v$ traversing $e_2$, using Lemma \ref{assgn:lem}, 
 it can be seen that $t=2c$, $a=c=0$, and $d(e_2)=d(e_1)$.  
 Let $2c=\delta$.
 At location $u$, we non-deterministically reset $c$; this reset 
 can be performed when  $a=4-\delta$, then 
 $t=\delta+(8-2\delta)=8-\delta$. 
 After $\frac{\delta}{2}$ elapse, we get $t=8, c=\frac{\delta}{2}, 
 a=4-\frac{\delta}{2}$. $t$ is reset. $a$ becomes 4 after $\frac{\delta}{2}$
 elapse; at this time, we have $c=t=\delta$. Thus, when $e_3$ is traversed, we have $c=\delta$
 and hence is doubled. The wrapping lemma gives us that $d(e_3+d(e_2)=d(e_1)$, and hence 
 is unchanged. 
 
 To increment $m$, we need to halve the value of $c$. This can be done in a manner similar to the above. 
\end{proof}

\begin{cor}
 For every $g >0$, $g \neq 1$, the reachability problem for hybrid systems with 
 \begin{itemize}
  \item One skewed clock with slope $g$, and any number of clocks,
  \item weak predicates
  \item variable-to-variable assignments 
 \end{itemize}
is undecidable.
\end{cor}
\begin{proof}
 After performing the assignment $t:=gc$ using the assignment lemma as in figure \ref{dec}, we 
 can use the variable-to-variable assignment $c:=t$ rather than guessing when to reset $c$ as done 
 in theorem \ref{thm:one}.
\end{proof}
\begin{cor}
\label{thm:three}
 The reachability problem of hybrid systems, with 
 \begin{itemize}
  \item clocks,
  \item weak doubling predicates with variable equality tests, 
  \item reset assignments
 \end{itemize}
is undecidable. 
\end{cor}

\begin{cor}
\label{thm:four}
The reachability problem of hybrid systems, with 
 \begin{itemize}
  \item clocks,
  \item weak addition predicates with variable equality tests, 
  \item reset assignments
 \end{itemize}
is undecidable. 
\end{cor}
An atomic weak doubling predicate is either an atomic  weak predicate or has the form $2x \leq c$ 
or $2x \geq c$ for $x \in V$. A weak doubling predicate is a conjunction of atomic weak doubling predicates. 
An atomic weak addition predicate is either an atomic  weak predicate or has the form $x+y \leq c$
or $x+y \geq c$ for $x,y \in V$. A  weak addition predicate is a conjunction of atomic weak addition predicates. 
 
 For doubling predicates, in fig \ref{dec}, replace the skewed clock $t$ with clock $t'$, and replace 
 occurrences of $t$ by $2t'$ in all enabling conditions. Replace resets of $t$ with resets of $t'$.
 Doubling predicates are a special case of addition predicates, hence theorems \ref{thm:three} and \ref{thm:four} follow.
 

 \begin{theorem}
  The reachability problem for hybrid systems with 
  \begin{itemize}
   \item one stopwatch, any number of clocks,
   \item weak predicates,
   \item reset assignments
  \end{itemize}
is undecidable.
 \end{theorem}
\begin{proof}
 The encoding of two counter machines is done as before. In figure \ref{sw}, we
 give a hybrid automaton that decrements counter $m$. It doubles the value of
 clock $c$ while maintaining the value of clock $d$, using two synchronization
 clocks $a,b$ and  a stopwatch variable $t$. To avoid clutter, we have omitted
 self loops of the form $d=4?, d:=0$ from the figure. 
 $t$ is such that $\dot{t}=1$ at $v_1,v_3,v_4,v_6$ and $\dot{t}=0$  at $v_2,v_5$.
 \input{doublingStop} 
  Let $\gamma=c(e_1)$ be the value of counter $m$ before decrementation. Location $v_1$ is an instance of 
  the assignment lemma, it performs the assignment $t:=c$. 
  Hence, we get $t(e_2)=c(e_2)=c(e_1)=\gamma$. Let $\delta=a(e_3)$ be the time elapse in location 
  $v_2$. Then we have $c(e_3)=c(e_2)+\delta=\gamma+\delta$, 
  $t(e_3)=t(e_2)=\gamma$, since $\dot{t}=0$ in $v_2$. Location $v_3$ is an instance of the equality lemma, 
  it checks whether $a$ and $t$ have the same value. 
  This means that $e_4$ can be traversed iff $\delta=\gamma$. Hence, $c(e_3)=\gamma+\delta=2\gamma$.
  Due to the wrapping lemma, we have $c(e_3)=c(e_4)=2 \gamma$. 
  The value of $d$ however, has changed and we need to maintain 
  the old value of $d$. Location $v_4$ is an instance of the assignment lemma, it performs 
  the assignment $t:=c$. Hence, we have $t(e_5)=c(e_5)=c(e_4)=2 \gamma$. 
  Since $\dot{t}=0$ in $v_5$, we have $t(e_6)=2 \gamma$. Location $v_6$ is another instance 
  of the assignment lemma, it performs the assignment $c:=t$. Thus, we have $c(e_7)=t(e_6)=2 \gamma$. Since $a=4$
  on coming out of $v_6$, and we have the self loop $d=4?d:=0$ on all locations, by wrapping we obtain 
  $d(e_7)=d(e_1)$.
  \end{proof}
\begin{theorem}
\label{thm:twoslope}
 For every $g >0$ with $g \neq 1$, the reachability problem for hybrid systems with 
 \begin{itemize}
 \item one two-slope variable with slopes 1 and $g$, and any number of clocks,
  \item weak predicates,
  \item reset assignments
 \end{itemize}
is undecidable.
\end{theorem}
\begin{proof}
 Assume $g=2$. Consider figure \ref{twoslope}. Doubling is done in figure \ref{twoslope}, 
 with a two slope variable $t$  with slopes 1,2. $dif(t,v)$ is such that 
 $\dot{t}=2$ and $dif(t,u)$ is such that 
 $\dot{t}=1$.  The location $v$ is an instance of the assignment lemma and performs the assignment $t:=2c$.
 The location $u$ is also an instance of the assignment lemma which performs the assignment $c:=t$.
 \input{doublingTwoSlope}
\end{proof}

\begin{cor}
 The reachability problem for linear hybrid automata with triangular differential inclusions 
 is undecidable.
\end{cor}
\begin{proof}
 The previous proof can be redone using linear variables $s,t$ and $u$ with slope $[1,2]$. The invariant 
 we maintain is $\dot{s} \leq \dot{t}  \leq \dot{u}$. The variable $t$ here corresponds to the two-slope 
 variable $t$ in theorem \ref{thm:twoslope}. To replicate the previous proof, we have to ensure that $\dot{t}=2$ 
 for the first 4 time units, and then $\dot{t}=1$ for the next 4 time units. 
 To ensure $\dot{t}=2$ for the first 4 time units, 
 we reset $s$ on the incoming edge (to $v$) and add the constraint $s=8$ on edge leading to $u$.  
 Similarly, to ensure that $\dot{t}=1$ for the second four time units, we 
 reset $u$ on the edge leading into $u$, and add the constraint $u=4$ on the edge coming out of $u$. 
\end{proof}

%\begin{theorem}
% \label{cerans}
% The reachability problem for hybrid systems with 
% \begin{itemize}
%  \item one memory cell, and any number of clocks,
%  \item weak predicates, 
%  \item variable-to-variable assignments
% \end{itemize}
% is undecidable. 
%\end{theorem}
%\begin{proof}
% The same encoding is used here as well. Figure \ref{cerans} 
% gives the doubling construction with one memory cell $u$ and 
% a clock $t$. 
%\input{doublingMemoryCell}
 
% The idea here is to store $c(e_1)$ in the memory cell $u$ using variable-to-variable assignment.
% A non-deterministic amount of time, $a(t_2)$ is spent in location $v_1$. 
% Let $\overline{x(e)}$ denote the value of variable $x$ on traversing $e$, after variable assignment has been made to $x$.
% As before, $x(e)$ denotes the value of variable $x$ on traversing edge $e$ before any variable assignment.
% Then, it can be seen that $\overline{c(e_3)}=\overline{u(e_2)}=c(e_2)=c(e_1)+a(e_2)$. To show that 
% $c(e_3)=2c(e_1)$, it suffices to show that $a(e_2)=c(e_1)$. The enabling condition of $e_3$ implies that 
% $\overline{a(e_2)}=\overline{t(e_2)}$. Hence, $a(e_2)=\overline{a(e_2)}=\overline{t(e_2)}=\overline{u(e_1)}=c(e_1)$.
% \end{proof}



 

